The S-matrix and boundary correlators in flat space

We consider the path integral of a quantum field theory in Minkowski spacetime with fixed boundary values (for the elementary fields) on asymptotic boundaries. We define and study the corresponding boundary correlation functions obtained by taking derivatives of this path integral with respect to the boundary values. The S-matrix of the QFT can be extracted directly from these boundary correlation functions after smearing. We interpret this relation in terms of coherent state quantization and derive the constraints on the path-integral as a function of boundary values that follow from the unitarity of the S-matrix. We then study the locality structure of boundary correlation functions. In the massive case, we find that the boundary correlation functions for generic locations of boundary points are dominated by a saddle point which has the interpretation of particles scattering in a small elevator in the bulk, where the location of the elevator is determined dynamically, and the S-matrix can be recovered after stripping off some dynamically determined but non-local ``renormalization'' factors. In the massless case, we find that while the boundary correlation functions are generically analytic as a function on the whole manifold of locations of boundary points, they have special singularities on a sub-manifold, points on which correspond to light-like scattering in the bulk. We completely characterize this singular scattering sub-manifold, and find that the corresponding residues of the boundary correlations at these singularities are precisely given by S-matrices. This analysis parallels the analysis of bulk-point singularities in AdS/CFT and generalizes it to the case of multi-bulk point singularities.

==> app_acm.tex <==
\section{Euclidean to Minkowski space}
In this appendix we obtain various foliations of the Minkowski space $\mathbb{R}^{d,1}$, by analytically continuing the Euclidean space $\mathbb{R}^{d+1}$. Consider the Cartesian coordinates on Euclidean space with metric
\begin{equation}\label{euclcyl}
    \begin{split}
        ds_E^2 &= (dX_E^0)^2 + \sum\limits_{i=1}^{d} (dX^i)^2.\\
        &= (dX_E^0)^2 + dr^2 + r^2 d\Omega_{d-1}^2
    \end{split}
\end{equation}
where, $r^2 = \sum_i X^iX^i$ and $d\Omega_{d-1}^2$ is the metric on $S^{d-1}$. We can view the Euclidean space as a foliation of constant $r$ surfaces. To obtain the Lorentzian space, we define
\begin{equation}
    t = - i  X_E^0,
\end{equation}
and obtain the standard Lorentzian metric
\begin{equation}
    \begin{split}\label{cylfoliation}
        ds^2 &= -dt^2 + r^2 d\Omega_{d-1}^2.
    \end{split}
\end{equation}
For the second foliation, consider the Euclidean metric in spherical coordinates.
\begin{equation}
    \begin{split}\label{euclpolar}
        ds_E^2 & = dR^2 + R^2 \, d\Omega^2_{d} \\
        & = dR^2 + R^2 \, ( d\theta^2 + \cos^2(\theta) \, d\Omega_{d-1}^2).
    \end{split}
\end{equation}
The coordinate $\theta$ ranges from $-\pi/2$ to $\pi/2$. The Euclidean space is foliated by constant $R$ surfaces. The coordinate $R$ is analogous to the proper distance in Lorentzian space. Define,
\begin{equation}
    \tau = - i \theta,
\end{equation}
the metric becomes,
\begin{equation}\label{dsfoliation}
    \begin{split}
        ds^2 &= d\rho^2 + \rho^2 \, ds^2_{dS_{d}}\\
        &= d\rho^2 + \rho^2 \, (-d \tau^2 + \cosh^2 \tau \, d\sph^2_{d-1}).
    \end{split}
\end{equation}
We have renamed $R$ to $\rho$, which is the more standard choice for the coordinate and is commonly used in the literature. Constant $\rho$ surface is a lower dimensional de-Sitter space. Note that these coordinates only cover the region outside the light cone emanating from $R=0$.

To obtain the region of Minkowski spacetime inside the light cone from \eqref{euclpolar}, we first note that R should be continued to proper time.\footnote{We are using same symbol for multiple coordinates. The coordinate $\tau$ defined below should not be confused with the one in de-Sitter foliation \eqref{dsfoliation}.}
\begin{equation}
    \begin{split}
        \tau = - i R.
    \end{split}
\end{equation}
The above continuation is not enough to get a Lorentzian metric as the resulting metric is completely time-like.
\begin{equation}
    \begin{split}
        ds^2 &= -d\tau^2 - \tau^2 \, ( d\theta^2 + \cos^2(\theta)  \, d\sph^2_{d-1})\\
        & = -d\tau^2 - \tau^2 \, ( \frac{d\chi^2}{1-\chi^2} + \chi^2  \, d\sph^2_{d-1}),
    \end{split}
\end{equation}
where we have introduced $\chi = \cos \theta$. Finally, consider the following transformation.
\begin{equation}
    \begin{split}
        \rho = - i \chi.
    \end{split}
\end{equation}
The metric becomes
\begin{equation}\label{adsfoliation}
    \begin{split}
        ds^2 &= -d\tau^2 + \tau^2 ds^2_{EAdS_d}\\
        ds^2_{EAdS_d} &= ( \frac{d\rho^2}{1+\rho^2} + \rho^2  \, d\sph^2_{d-1}).
    \end{split}
\end{equation}
This is the Euclidean-AdS foliation of the the region of Minkowski space inside the light cone emanating from the origin.

==> app_example.tex <==
\section{S-matrix from Euclidean correlations - An example}\label{app_example}
The goal of this appendix is to relate Euclidean correlation function of a massive (real) scalar field to S-matrix elements. To begin, we first note that the free scalar field admits the following expansion in Minkowski space.
\begin{equation}
    \begin{split}
        \Phi(x) = \int {d^d \Vec{k} \over (2\pi)^{d/2}} {1\over \sqrt{2 \omega_{\Vec{k}}}} \left( a(\Vec{k})e^{i k.x} + h.c.  \right), \qquad \omega_{\Vec{k}} = \sqrt{|\Vec{k}|^2 + m^2}.
    \end{split}
\end{equation}
Canonical commutation relations imply,
\begin{equation}
    [a(\Vec{k}_1),a^{\dagger}(\Vec{k}_2)] = \delta^d(\Vec{k}_1 - \Vec{k}_2).
\end{equation}
We allow interactions, which we will specify as and when needed. We assume that even in presence of interactions, the scalar field satisfies free equations of motion at asymptotically early and late times. This suggests that we can define following expansions of the scalar field.
\begin{equation}
    \begin{split}
        \Phi(x) &= \int {d^d \Vec{k} \over (2\pi)^{d/2}} {1\over \sqrt{2 \omega_{\Vec{k}}}} \left( a_{in}(\Vec{k}) \phi^{in}_{\Vec{k}}(x) + h.c.  \right)\\
        &= \int {d^d \Vec{k} \over (2\pi)^{d/2}} {1\over \sqrt{2 \omega_{\Vec{k}}}} \left( a_{out}(\Vec{k}) \phi^{out}_{\Vec{k}}(x) + h.c.  \right),
    \end{split}
\end{equation}
where the ``in" and ``out" modes asymptote to plane waves at early and late times respectively.
\begin{equation}
    \begin{split}
        \lim\limits_{t \rightarrow -\infty} \phi^{in}_{\Vec{k}}(x) &= e^{ik.x}\\
        \lim\limits_{t \rightarrow \infty} \phi^{out}_{\Vec{k}}(x) &= e^{ik.x}.
    \end{split}
\end{equation}
The operators $a_{in}$ and $a_{out}$ independently satisfy canonical commutation relations.
\begin{equation}
    \begin{split}
        [a_{in}(\Vec{k}_1),a_{in}^{\dagger}(\Vec{k}_2)] &= \delta^d(\Vec{k}_1 - \Vec{k}_2)\\
        [a_{out}(\Vec{k}_1),a_{out}^{\dagger}(\Vec{k}_2)] &= \delta^d(\Vec{k}_1 - \Vec{k}_2).
    \end{split}
\end{equation}
The non-trivial relation between $a_{in}$ and $a_{out}$ is encoded in the S-matrix and depends on the details of interactions.


\subsection*{S-matrix as a correlation function in position space}
Let us first evaluate the scalar field at very late times.
\begin{equation}\nonumber
    \begin{split}
        \lim\limits_{T\rightarrow\infty} \Phi(T, {\Vec{p} \, T \over \sqrt{|\Vec{p}|^2 + m^2}}) = \lim\limits_{T\rightarrow\infty} \int {d^d \Vec{k} \over (2\pi)^{d/2}} {1\over \sqrt{2 \omega_{\Vec{k}}}}  a_{out}(\Vec{k}) e^{-iT\left(\sqrt{|\Vec{k}|^2 + m^2} - {\Vec{p}.\Vec{k} \over \sqrt{|\Vec{p}|^2 + m^2}}\right)} + h.c. 
    \end{split}
\end{equation}
Using saddle point approximation, we get \PS{check coefficients}
\begin{equation}
    \lim\limits_{T\rightarrow\infty} \Phi(T, {\Vec{p} \, T \over \sqrt{|\Vec{p}|^2 + m^2}}) = a_{out}(\Vec{p}\,) {e^{-imT/\omega_{\Vec{p}}} \over \sqrt{2 \omega_{\Vec{p}}}} + h.c.
\end{equation}
This expression simplifies if we consider the E-AdS foliation of Minkowski space \eqref{adsfoliation}.
\begin{equation}
    \lim\limits_{\tau \rightarrow\infty} \Phi(\tau,\rho=|\vec{p}\,|/m,\sph=\hat{p}) = {e^{-im\tau} \over 2 \sqrt{\omega_{\vec{p}}}} a_{out} (\vec{p}\,) + h.c.
\end{equation}
Similar relation holds for ``in" modes. 
\begin{equation}
    \lim\limits_{\tau \rightarrow -\infty} \Phi(\tau,\rho=|\vec{p}\,|/m,\sph=-\hat{p}) = {e^{im\tau} \over 2 \sqrt{\omega_{\vec{p}}}} a_{in} (\vec{p}\,) + h.c.
\end{equation}
Hence, the S-matrix can be evaluated by considering correlation functions with excitations localized on early and late time E-AdS slices. To see this explicitly, consider an S-matrix element 
\begin{equation}
    \begin{split}
        G(p_1,\cdots , p_n) = \prod\limits_i {1 \over p_i^2 + m^2 - i\epsilon} S(p_1,\cdots , p_n) + \cdots
    \end{split}
\end{equation}
where the ellipsis represent disconnected pieces. We evaluate its Fourier transform at asymptotic points.
\begin{equation}\label{sgeuc}
    \begin{split}
        \lim\limits_{\tau_i\rightarrow\infty} G(\tau_i,\vec{k}_i/m) = \prod\limits_i \lim\limits_{\tau_i\rightarrow\infty} \left. \int d^4 p_i {1\over p_i^2 + m^2 - i\epsilon} S(p_i) e^{- i p_i . x_i} \right|_{x_i=(\tau_i,\vec{k}_i)}
    \end{split}
\end{equation}
If the leading contribution comes from poles $p_i^2+m^2-i\epsilon$, then the above Fourier transform results in
\begin{equation}\label{smatrixtocorrpos}
    \lim\limits_{\tau_i\rightarrow\infty} G(\tau_i,\vec{k}_i/m) = \# S(k_i).
\end{equation}
\PS{coefficient needs to be fixed. Also, should we expand the presentation by including insertions in the past?}

To summarize, the connected piece of the S-matrix with an outgoing particles of momentum $p_i$ can be obtained by considering time ordered correlation functions with insertions localized in the far future EAdS slice. Location of the insertions is the point of intersection of the classical trajectories of a particles carrying the momenta $p_i$ and the asymptotic slice.

\subsection*{S-matrix from Euclidean correlations}
\PS{Additional comments about analyticity of correlation functions?}
Lorentzian time-ordered correlation functions can be obtained via following analytic continuation of the Euclidean correlation functions.
\begin{equation}
    \begin{split}\label{analyticcont_eucl_corr-scattering}
        \langle {\cal T} \Phi(t_1,\vec{x}_1) \cdots  \Phi(t_n, \vec{x}_n) \rangle = \lim\limits_{\epsilon \rightarrow 0} \, \langle  \Phi(\tau = (\epsilon + i )t_1,\vec{X}_1) \cdots \Phi(\tau = (\epsilon + i )t_n, \vec{X}_n) \rangle,
    \end{split} 
\end{equation}
where $\tau = it $ is the Euclidean time coordinate. Combined with \eqref{smatrixtocorrpos}, this suggests a relation between Euclidean correlation functions and S-matrix that we now verify in perturbation theory.
\subsubsection*{4-point function - contact diagram}
\begin{figure}
    \centering
    \includegraphics[height=0.3\textheight]{graphics/E4ptcontact.png}
    \caption{Contact diagram - contribution to 4-point function}
    \label{fig:4ptcontact}
\end{figure}
First, let us consider the correction to 4-point function due to a $\phi^4$ contact interaction. The corresponding S-matrix is simply a total momentum conserving delta-function.
\begin{equation}
    S_{contact}(p_1,p_2,p_3,p_4) = \delta^4(p_1+p_2+p_3+p_4).
\end{equation}
The correction to the Euclidean correlation function is given by a contact diagram Fig. \ref{fig:4ptcontact}.
\begin{equation}
    \begin{split}
        G_{E,contact}(x_1,x_2,x_3,x_4) = \int dx \, G_E(x_1,x)G_E(x_2,x)G_E(x_3,x)G_E(x_4,x),
    \end{split}
\end{equation}
where $X_i$ are ``boundary" insertions and $G_E(x,y)$ is the free Euclidean propagator between points $x$ and $y$. On the propagator, we impose the boundary condition
\begin{equation*}
    \lim\limits_{|x-y|\rightarrow \infty} G_E(x,y) = 0.
\end{equation*}
% \PS{To do - solve for propagator, show large distance behavior, compute the diagram}
The free Euclidean propagator satisfying the above boundary condition is
\begin{equation}\label{propagatoreuclfree}
    G_E(x,y) = {K_{d-1\over 2}(m \, |x-y|) \over |x-y|^{d-1 \over 2}}.
\end{equation}
We require the propagator in the limit when one of the insertion is large, say, $y=\Lambda Y$, such that $Y^2$ is finite. Expanding the geodesic distance asymptotically in $\lambda$.
\begin{equation}
    \begin{split}
        |x-y| &= \left(x^2 + \Lambda^2 Y^2 - 2 \Lambda x \cdot Y\right)^{1/2}\\
        &= \Lambda Y \left( 1 - 2 {x \cdot Y \over \Lambda Y^2} + {x^2 \over \Lambda^2 Y^2} \right)^{1/2}\\
        &= \Lambda Y - {x \cdot Y \over Y} +  {x^2 \over 2 \Lambda Y} + {(x\cdot y)^2 \over 2 \Lambda Y^3} + O(\Lambda^{-2})\\
        &= \Lambda Y - x \cdot \hat{Y} +  {x^2 + (x\cdot \hat{Y})^2  \over 2 \Lambda Y} + O(\Lambda^{-2}),
    \end{split}
\end{equation}
where we have defined a unit vector, $\hat{Y}^2 = 1$. In this limit, the propagator decays to zero exponentially.
\begin{equation}
    \begin{split}
        G_{E}(x,\Lambda Y) \sim {e^{- m \left(\Lambda Y^2 - x \cdot \hat{Y} +  {x^2 + (x\cdot \hat{Y})^2  \over 2 \Lambda Y} \right)} \over (\Lambda Y)^{d/2}}
    \end{split}
\end{equation}
Substituting in the integral for correction to the 4-point function due to contact diagram.
\begin{equation}
    \begin{split}
        G_{E,contact}(x_1,x_2,x_3,x_4) = \left[ \prod\limits_{i=1}^4 \,  { e^{-m \, \Lambda \, X_i } \over (\Lambda \, X_i)^{d/2} } \right]  \int dx \, e^{m \, x \cdot (\hat{X}_1 + \hat{X}_2 +\hat{X}_3 +\hat{X}_4) } 
    \end{split}
\end{equation}
To get the above expression, we have ignored the terms in the exponential that scales with $\Lambda^{-1}$. Clearly, this is justified as long as $x$ doesn't scale with $\Lambda$. This will be true if the interactions are localized away from the boundary. However, let us try to estimate the contribution from large $x = \Lambda X$. Since the geodesic distance scales with $\Lambda$, unless x is close to a boundary insertion, the Bessel function would decay. Schematically, we can write the contribution as (after scaling with the extrapolate factor)
\begin{equation}
    \begin{split}
        \lim\limits_{\Lambda\rightarrow\infty} \int \Lambda^{d+1}\, d^{d+1} X\, {e^{-m\,\Lambda\, \sum ( |X-X_i| - X_i )} \, X_i^{d/2} \over \, |X-X_i|^{d/2} } 
    \end{split}
\end{equation}
The above integral diverges due to contribution from the region $ |X-X_i| - X_i < 0$. This suggests the S-matrix would be finite only if interactions are turned off at large distances. The above divergence leads to subtlety in defining the extrapolate dictionary relating the scalar field to a boundary operator.

For now, we assume that the interactions are indeed switched off at large distances. To obtain the S-matrix, we need to analytically continue the above integral following \eqref{analyticcont_eucl_corr-scattering}.
\begin{equation}
    \begin{split}
        X_i &= x(p_i) = \left( (\epsilon + i) T, {\vec{p}_i \, T \over \sqrt{|\Vec{p}_i|^2 + m^2}} \right)\\
        \Lambda X_i & = \sqrt{x^2} = {T \over E_{p_i}} \sqrt{(i+\epsilon)^2 E_{p_i}^2 + |\vec{p}|^2} = {T \over E_{p_i}} \sqrt{-m^2 + i \epsilon},
    \end{split}
\end{equation}
where $E_{p}^2 = |\vec{p}|^2 + m^2 $. The ambiguity in the phase due to square root is removed by the $i\epsilon$. The function $f(x)=\sqrt{x+i\epsilon}$ is analytic in upper half of complex $x$ plane if we extend the branch cut in lower half plane. So, $f(-|x|) = f(e^{i\pi} |x| ) = e^{i \pi/2} |x|$. Using this, we can write
\begin{equation}
    \begin{split}
        \Lambda X_i &= {i\, m\, T \over E_{p_i}}\\
        \hat{X_i} &= {x(p_i) \over \Lambda X_i} =  {1\over m}(E_{p_i}(1 - i \epsilon), -i \vec{p}_i), 
    \end{split}
\end{equation}
Substituting in the integral for contact diagram, we get
\begin{equation}
    \begin{split}
         G_{E,contact}(x(p_i)) = \left[ \prod\limits_{i=1}^4 \,  { e^{-i m^2 T\over E_{p_i}} \over ({i m T\over E_{p_i}})^{d/2}  } \right]  \int dt_E\, d\vec{x} \, e^{ - i \vec{x} \cdot \sum \vec{p}_i } \, e^{t_E \sum (1 - i \epsilon) E_{p_i}}
    \end{split}
\end{equation}
